Domain-wall dynamics in translationally noninvariant nanowires: theory and applications

We generalize domain-wall dynamics to the case of translationally noninvariant ferromagnetic nanowires. The obtained equations of motion make the description of the domain-wall propagation more realistic by accounting for the variations along the wire, such as disorder or change in the wire shape. We show that the effective equations of motion are very general and do not depend on the model details. As an example of their use, we consider an hourglass-shaped nanostrip in detail. A transverse domain wall is trapped in the middle and has two stable magnetization directions. We study the switching between the two directions by short current pulses. We obtain the exact time dependence of the current pulses required to switch the magnetization with the minimal Ohmic losses per switching. Furthermore, we find how the Ohmic losses per switching depend on the switching time for the optimal current pulse. As a result, we show that as a magnetic memory this nanodevice can be $10^5$ times more energy efficient than the best modern devices.

==> PaxHeader/nontranslational_DWdyn.tex <==
30 ctime=1315977006.104336325
30 atime=1315977129.416719617
20 SCHILY.dev=64770
22 SCHILY.ino=1311267
18 SCHILY.nlink=1
88 LIBARCHIVE.xattr.security.selinux=dW5jb25maW5lZF91Om9iamVjdF9yOnVzZXJfaG9tZV90OnMwAA

